Feature Averaging: An Implicit Bias of Gradient Descent Leading to Non-Robustness in Neural Networks

In this work, we investigate a particular implicit bias in gradient descent training, which we term "Feature Averaging," and argue that it is one of the principal factors contributing to the non-robustness of deep neural networks. We show that, even when multiple discriminative features are present in the input data, neural networks trained by gradient descent tend to rely on an average (or a certain combination) of these features for classification, rather than distinguishing and leveraging each feature individually. Specifically, we provide a detailed theoretical analysis of the training dynamics of two-layer ReLU networks on a binary classification task, where the data distribution consists of multiple clusters with mutually orthogonal centers. We rigorously prove that gradient descent biases the network towards feature averaging, where the weights of each hidden neuron represent an average of the cluster centers (each corresponding to a distinct feature), thereby making the network vulnerable to input perturbations aligned with the negative direction of the averaged features. On the positive side, we demonstrate that this vulnerability can be mitigated through more granular supervision. In particular, we prove that a two-layer ReLU network can achieve optimal robustness when trained to classify individual features rather than merely the original binary classes. Finally, we validate our theoretical findings with experiments on synthetic datasets, MNIST, and CIFAR-10, and confirm the prevalence of feature averaging and its impact on adversarial robustness. We hope these theoretical and empirical insights deepen the understanding of how gradient descent shapes feature learning and adversarial robustness, and how more detailed supervision can enhance robustness.

==> Averaging.tex <==
\section{Feature Averaging and Non-robustness}
\label{sec:landscape}

\kaifeng{the whole section will be removed}

%In this section, we illustrate how the phenomenon of feature average hurts robustness by giving some constructed neural networks. Note that we are by default working with a binary classification task if not specified. We first provide the following feature averaging example.
%In this section, we demonstrate how the feature averaging phenomenon can adversely affect robustness through several specifically constructed neural networks. Unless otherwise specified, we assume a binary classification task by default.

As a warm-up, here we present two distinct parameter regimes for our two-layer network learner: \textit{feature averaging} and \textit{feature decoupling}. 
The former means the weights associated with each neuron is a linear average of features, while the latter indicates that distinct features will be learned by separate neurons.
Our construction is similar to that in \citet{frei2024double} and \citet{min2024can}. \kaifeng{when you say something of yours is similar to someone else's, it is good to say what is different soon after}
We illustrate how a feature averaging solution leads to non-robustness,
while a feature decoupling solution is more robust (w.r.t. to a much larger robust radius) in $\Dbinary$.

Now, we begin by presenting the following example of feature-averaging two-layer neural network.
%\binghui{Frei2024 doesn't give explicit construction?}
%by giving some constructed neural networks.

%Now, we begin by presenting the following example of feature-averaging two-layer neural network.

\textbf{Feature-Averaging Two-Layer Neural Network.} Consider the following two-layer neural network,
in which the weights associated with each neural is the average of many feature $\boldsymbol{\mu}_j$'s.
Since we have identical positive neurons and identical negative neuron,
the network can be simplified as (i.e., we merge identical neurons as one neuron):
\begin{equation}
    f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}) := \underbrace{\operatorname{ReLU}\bigg(\bigg\langle \sum_{j\in  J_{+}}\boldsymbol{\mu}_j, \boldsymbol{x}\bigg\rangle + b_{+}\bigg)}_{\textit{deals with all positive clusters}} - \underbrace{\operatorname{ReLU}\bigg(\bigg\langle \sum_{j\in  J_{-}}\boldsymbol{\mu}_j, \boldsymbol{x}\bigg\rangle + b_{-}\bigg)}_{\textit{deals with all negative clusters}} , \nonumber
\end{equation}
where we choose weight $\boldsymbol{w}_{s,r} = \sum_{j\in J_{s}}\boldsymbol{\mu}_j$ and bias $b_{s,r} = b_s$ for $s\in\{-1,+1\},r\in[m]$.

Indeed, the feature-averaging network uses the first neuron to process all data within positive clusters, and it uses the second neuron to process all data within negative clusters. Thus, it can correctly classify clean data, which is shown as the following proposition.

\begin{proposition}[Feature-averaging network can achieve nearly perfect standard accuracy]
\label{prop:warm_up_avg_acc}

    There exist values of $b_{+}$ and $b_{-}$ such that the feature-averaging network $f_{\boldsymbol{\theta}_{\textit{avg}}}$ achieves $1-o(1)$ standard accuracy over $\Dbinary$.
\end{proposition}

Actually, it can be easily checked by choosing $b_{+}=b_{-}=0$. Proposition \ref{prop:warm_up_avg_acc} manifests that only two-neuron network with feature-averaging weights is able to classify binary classes perfectly. However, it fails to robustly classify perturbed data whatever the bias term is chosen, which is shown as:

\begin{proposition}[Feature averaging leads to non-robustness]
\label{prop:warm_up_avg_robust}

    %For any values of $b_{+}$ and $b_{-}$ such that $f_{\boldsymbol{\theta}_{\textit{avg}}}$ has 1-o(1) standard accuracy , it holds that the feature-averaging network $f_{\boldsymbol{\theta}_{\textit{avg}}}$ has at most $\frac{c}{1+c}$ $\delta-$robust accuracy for arbitrary perturbation radius $\delta = \omega(\sqrt{d/k})$.
    For any values of $b_{+}$ and $b_{-}$ such that $f_{\boldsymbol{\theta}_{\textit{avg}}}$ has $1 - o(1)$ standard accuracy, it holds that the feature-averaging network $f_{\boldsymbol{\theta}_{\textit{avg}}}$ has zero $\delta-$robust accuracy for perturbation radius $\delta = \Omega(\sqrt{d/k})$.
\end{proposition}

\textbf{Proof Intuition.} In fact, the attack can be chosen as $\boldsymbol{\rho} \propto -\sum_{j\in J_{+}} \boldsymbol{\mu}_j + \sum_{l\in J_{-}}\boldsymbol{\mu}_l$ and $\|\epsilon\| = \delta$, which is both universal \citep{zhang2021survey} and transferable \citep{papernot2016transferability}. Intuitively, for averaged features $\boldsymbol{w}_{s,r} = \sum_{j\in J_{s}}\boldsymbol{\mu}_j$, this perturbation can activate almost all of ReLU neurons, which leads a linear approximation $f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x} + \boldsymbol{\rho}) \approx f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}) + \langle \nabla_{\boldsymbol{x}}f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}), \boldsymbol{\rho}\rangle$. Since $f_{\boldsymbol{\theta}_{\textit{avg}}}$ has $1 - o(1)$ standard accuracy, we know that the classifier achieves a positive margin, i.e. $0 < y f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}) \leq O(d)$ w.h.p. over $(\boldsymbol{x}, y)$ sampled from $\Dbinary$. Then, due to a large gradient norm over data input, i.e. $\|\nabla_{\boldsymbol{x}}f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x})\| \approx \|\sum_{j\in J_{+}} \boldsymbol{\mu}_j - \sum_{l\in J_{-}}\boldsymbol{\mu}_l\| = \Omega(\sqrt{k d})$, we derive that the feature-averaging network $f_{\boldsymbol{\theta}_{\textit{avg}}}$ has zero $\delta-$robust accuracy for perturbation radius $\delta = \Omega(\sqrt{d/k})$.


%\begin{definition}
%    We call the neural network as a feature average solution when $w_j=\dfrac{1}{d}\sum\limits_{y^{(i)}=y^{(j)}}\mu ^{(i)}$. Specifically, it's in the form of 
%    $$
%\mathcal{N}_{avg}(\mathbf{x})= \dfrac{1}{\sqrt{m}} \sum_{y^{(j)}=1}\phi\left(\left(\dfrac{1}{d}\sum\limits_{y^{(i)}=1}\mu ^{(i)}\right)^{\top} \mathbf{x}+b_j\right)- \dfrac{1}{\sqrt{m}}\sum_{y^{(j)}=-1} \phi\left(\left(\dfrac{1}{d}\sum\limits_{y^{(i)}=-1}\mu ^{(i)}\right)^{\top} \mathbf{x}+b_j\right). 
%$$
%\end{definition}
%\begin{theorem}
%    For any choice of $b_{+}$ and $b_{-}$ s.t. $f_{\textit{avg}}$ is a useful feature  but it is not $\sqrt{d}$-robust.
    
%    (It is $\sqrt{d/k}$-robust).
%\end{theorem}

% \begin{proof_sketch}
% \label{proof_sketch_prop:warm_up_avg_robust}
% We use proof by contradiction. 



%  For $x_1\in  J^+, x_2\in \mathcal{J^-}$, 
%   $   f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}_1)-f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}_2) \le 2d$.

%   So $\textbf{max}\{f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}_1), -f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}_2)\}\le 2d$.
% Then we can use $\delta=\dfrac{8}{k}\sum\limits_{i\in [k]}y_i\mu_i$ to attack $f_{\theta_{\textit{avg}}}$ 

% Since
% $\bigg\langle \sum_{j\in  J_{+}}\boldsymbol{\mu}_j, -\delta \bigg\rangle \approx -4d,\bigg\langle \sum_{j\in  J_{-}}\boldsymbol{\mu}_j, -\delta \bigg\rangle \approx 4d$,  so $f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}_1-\delta)\le 0$, $f_{\boldsymbol{\theta}_{\textit{avg}}}(\boldsymbol{x}_2-\delta) \ge 0$
% \end{proof_sketch}

% Proof sketch: Comparing $f_{\textit{avg}}(\boldsymbol{x}-\boldsymbol{\mu}_i+\boldsymbol{\mu}_j)$ and $f_{\textit{avg}}(\boldsymbol{x}-\dfrac{2}{k}\sum\limits y_i\boldsymbol{\mu}_i)$.

%\kaifeng{better name? Maybe we could call them feature-averaged solution v.s.~feature-disentangled solution}

Proposition \ref{prop:warm_up_avg_robust} shows that the feature-averaging solution has a poor robust performance due to a universal attack that aligns with the negative direction of the label-weighted average of cluster features. In contrast to the feature averaging regime, we consider an alternative regime as known feature decoupling as follows.

\textbf{Feature-Decoupling Two-Layer Neural Network.} In the feature decoupling regime, we present the following network construction with $k$ neurons:
\begin{equation}
    f_{\boldsymbol{\theta}_{\textit{dec}}}(\boldsymbol{x}):=\frac{1}{m}\sum_{j\in J_{+}}\underbrace{\operatorname{ReLU}\left(\langle \boldsymbol{\mu}_j, \boldsymbol{x}\rangle + b_j^{+} \right)}_{\textit{deals with positive cluster }j} - \frac{1}{m}\sum_{l\in J_{-}}\underbrace{\operatorname{ReLU}\left(\langle \boldsymbol{\mu}_l, \boldsymbol{x}\rangle + b_l^{-}\right)}_{\textit{deals with negative cluster }l}, \nonumber
\end{equation}
where we choose weight $\boldsymbol{w}_{s,r} = \boldsymbol{\mu}_{r}$ and $b_{s,r} = b_{r}^{s}$ for $s\in\{-1,+1\}, r\in \{1,2,\dots,|J_{s}|\}$, and $\boldsymbol{w}_{s,r} = \boldsymbol{0}$ and $b_{s,r} = 0$ for other index pair $(s,r) \in \{-1,+1\}\times[m]$.

We show that the feature-decoupling network is more robust to perturbations, which is presented as:

\begin{proposition}[Achieving robustness via feature decoupling]
\label{prop:warm_up_dec_robust}
    There exists values of $b_j^{+},b_l^{-}$ such that the feature-decoupling network $ f_{\boldsymbol{\theta}_{\textit{dec}}}$ has $1-o(1)$ $\delta-$robust accuracy for radius $\delta = O(\sqrt{d})$.%, which also achieves nearly-optimal robustness under our setting. 
\end{proposition}


\iffalse
\begin{proof_sketch}
\label{proof_sketch_prop:warm_up_dec_robust}
Consider $b_j=-d/2$.  For $x\in I_j,$
$\langle \boldsymbol{\mu_i}, \boldsymbol{x}\rangle +b_i \begin{cases}
\ge & \ \ d/4 \ \ \ \ \ i=j\\
\le & -d/4 \ \ \ \ i\ne j    
\end{cases}$

For any perturbation $\delta$ such that $\|\delta\|=\sqrt{d}/8.$

We still have $\langle \boldsymbol{\mu_i}, \boldsymbol{x}-\delta\rangle +b_i \begin{cases}
\ge & \ \ d/8 \ \ \ \ \ i=j\\
\le & -d/8 \ \ \ \ i\ne j    
\end{cases}$
So $f_{\boldsymbol{\theta}_{\textit{dec}}}$ has $1-o(1)$ $\delta-$robust accuracy for any robust radius $\delta = O(\sqrt{d})$. 
\end{proof_sketch}
\fi

%Proposition \ref{prop:warm_up_avg_robust} and Proposition \ref{prop:warm_up_dec_robust} illustrate that for two-layer neural networks with the same architecture, there exist different feature learning regimes, corresponding to non-robust solutions, which inspires us exploring feature learning process of gradient descent in order to understand non-robustness in trained neural networks.

\textbf{Proof Intuition.} For decoupled features, each neuron deals with one certain positive cluster $j$ (or negative cluster $l$), and we also apply the bias term $b_{j}^{+} = b_{l}^{-} = -\frac{\sqrt{d}}{2}$ to filter out intra/inter cluster noise. In this regime, for each data point $(\boldsymbol{x},y)$ belonging to cluster $i$ (we assume cluster $i$ is a positive cluster and $y = 1$) and perturbation $\boldsymbol{\rho}$ ($\|\boldsymbol{\rho}\|\leq \delta$), we have the following linearization, w.h.p. $f_{\boldsymbol{\theta}_{\textit{dec}}}(\boldsymbol{x}+\boldsymbol{\rho}) \approx \frac{1}{m} \langle \boldsymbol{\mu}_i, \boldsymbol{x}+\boldsymbol{\rho}\rangle$. Then, we know $ f_{\boldsymbol{\theta}_{\textit{dec}}}$ has $1-o(1)$ $\delta-$robust accuracy for $\delta = O(\sqrt{d})$.

\begin{remark}[Optimality]
    Indeed, one can easily verify that $f_{\boldsymbol{\theta}_{\textit{dec}}}$ achieves optimal robustness since the distance between distinct cluster centers is at most $\Theta(\sqrt{d})$ (i.e. $\|\boldsymbol{\mu}_i-\boldsymbol{\mu}_j\| = \Theta(\sqrt{d}), \forall i\ne j$).
\end{remark}

We give the full proofs of Proposition \ref{prop:warm_up_avg_acc}, \ref{prop:warm_up_avg_robust} and \ref{prop:warm_up_dec_robust} in Appendix \ref{appendix:warm_up}. Proposition \ref{prop:warm_up_avg_robust} and Proposition \ref{prop:warm_up_dec_robust} illustrate that for two-layer neural networks of the same architecture, different feature learning regimes exist. These regimes correspond to non-robust solutions and robust solutions, respectively. This observation inspires us to explore the \textit{feature learning process} of gradient descent in order to understand the origins of non-robustness in trained neural networks.

%\textbf{Feature Individual Solution.}

%\begin{equation}
%    f_{\textit{ind}}(\boldsymbol{x}):= \sum_{j\in J_{+}}\operatorname{ReLU}(\langle \boldsymbol{\mu}_j, \boldsymbol{x}\rangle + b_j) - \sum_{j\in J_{-}}\operatorname{ReLU}(\langle \boldsymbol{\mu}_j, \boldsymbol{x}\rangle + b_j) . \nonumber
%\end{equation}

%\begin{definition}
%    We call the neural network as a feature individual solution when $w_j=\dfrac{1}{d}\mu ^{(j)}$. 
    
%    Specifically, it's in the form of 
%$$
%\mathcal{N}_{ind}(\mathbf{x})=\sum_{y^{(j)}=1} \dfrac{1}{\sqrt{m}} \phi\left(\dfrac{1}{d}\mu^{(j)\top} \mathbf{x}+b_j\right)- \sum_{y^{(j)}=-1} \dfrac{1}{\sqrt{m}} \phi\left(\dfrac{1}{d}{}\mu^{(j)\top} \mathbf{x}+b_j\right).
%$$
%\end{definition}
%\begin{theorem}
%    There exists a choice of $b_j,j\in [k]$ s.t. $f_{\textit{ind}}$ is a useful feature and it is also $\sqrt{d}$-robust.
%\end{theorem}

%Proof sketch: $b_j=-d/2$.
